Bootstrapping Networks with Latent Space Structure

A core problem in statistical network analysis is to develop network analogues of classical techniques. The problem of bootstrapping network data stands out as especially challenging, since typically one observes only a single network, rather than a sample. Here we propose two methods for obtaining bootstrap samples for networks drawn from latent space models. The first method generates bootstrap replicates of network statistics that can be represented as U-statistics in the latent positions, and avoids actually constructing new bootstrapped networks. The second method generates bootstrap replicates of whole networks, and thus can be used for bootstrapping any network function. Commonly studied network quantities that can be represented as U-statistics include many popular summaries, such as average degree and subgraph counts, but other equally popular summaries, such as the clustering coefficient, are not expressible as U-statistics and thus require the second bootstrap method. Under the assumption of a random dot product graph, a type of latent space network model, we show consistency of the proposed bootstrap methods. We give motivating examples throughout and demonstrate the effectiveness of our methods on synthetic data.

==> apx_gen_sparse.tex <==
We begin by collecting a handful of technical results from the existing
literature on random dot product graphs that will be useful in
the proofs below.

\begin{lemma}
\label{lem:rdpgfacts}
Let $(A,X) \sim \RDPG(F,n)$ for some $d$-dimensional inner product
distribution $F$.
Define $P = X X^T \in \bbR^{n \times n}$ so that
$\E[ A \mid X] = P$ and let
$\UP \SP \UP^T$ be the rank-$d$ eigendecomposition of $P$,
so that $\SP \in \bbR^{d \times d}$ is a diagonal matrix with entries
given by the eigenvalues
$\lambda_1(P) \ge \lambda_2(P) \ge \dots \ge \lambda_d(P) > 0$
and $\UP \in \bbR^{n \times d}$ has as its columns the $d$ corresponding
unit eigenvectors.
Similarly, let $\UA \SA \UA^T = \Xhat \Xhat^T \in \bbR^{n \times n}$
be the rank-$d$ approximation of
$A$ given by its top $d$ largest-magnitude eigenvalues and eigenvectors.
That is, let $\SA \in \bbR^{d \times d}$ be the diagonal matrix
with entries given by the $d$ largest-magnitude eigenvalues of $A$
and let $\UA \in \bbR^{n \times d}$
have as its columns the $d$ corresponding unit eigenvectors.
There exist constants $C_2 \ge C_1 > 0$ such that
with probability at least $1-Cn^{-2}$,
%[Adapted from \cite{LevAthTanLyzYouPri2017}, Observations 1 and 2]
\begin{equation} \label{eq:specgrowth:1}
C_1 n \le \lambda_d(P) \le \dots \le \lambda_1(P) \le C_2 n
\end{equation}
\begin{equation} \label{eq:specgrowth:2}
\text{ and } \| A - P \| \le C \sqrt{n \log n}.
%log factor is correct. See https://arxiv.org/pdf/0911.0600.pdf and/or https://projecteuclid.org/download/pdfview_1/euclid.ejs/1420815881 pg 9
\end{equation}
Further, letting $Q \in \bbR^{d \times d}$
be the orthogonal matrix guaranteed by Lemma~\ref{lem:2toinfty},
for all suitably large $n$ it holds with probability at least
$1-Cn^{-2}$ that
%[Adapted from \cite{lyzinski15_HSBM}, Proposition 16]
\begin{equation} \label{eq:innerprod} %\label{lem:innerprod}
\| Q - \UA^T \UP \|_F \le Cn^{-1} \log n, %TODO: check log.
\end{equation}
%\begin{lemma}[Adapted from \cite{lyzinski15_HSBM} Lemma 17]
\begin{equation} \label{eq:Qswap} %\label{lem:Qswap}
\| Q \SA^{-1/2} - \SP^{-1/2} Q \|_F \le C n^{-3/2},
%No log factor because they use Lu and Peng. we need a log-factor if we want to avoid that.
\end{equation}
%[Adapted from \cite{LevAthTanLyzYouPri2017}, Lemma 5]
\begin{equation} \label{eq:DKmodified} %\label{lem:DKmodified}
\| \UA Q - \UP \|_F \le \frac{ C \log^{1/2} n }{ \sqrt{n} }.
%log-factor agrees with eq:specgrowth.
\end{equation}
\end{lemma}
\begin{proof}
Equations~\eqref{eq:specgrowth:1} and~\eqref{eq:specgrowth:2}
are Observations 1 and 2, respectively, in
\cite{LevAthTanLyzYouPri2017}.
Equations~\eqref{eq:innerprod} and~\eqref{eq:Qswap} follow from,
respectively, Proposition 16 and Lemma 17 in \cite{lyzinski15_HSBM}.
A proof of Equation~\eqref{eq:DKmodified} appears in the course of
the proof of Lemma 5 in \cite{LevAthTanLyzYouPri2017}.
%% https://arxiv.org/pdf/1705.09355.pdf
We restate it here for the sake of completeness.

By Theorem 2 in \cite{YuWanSam2015},
there exists orthonormal $Q \in \bbR^{d \times d}$ such that
\begin{equation*}
\| \UA Q - \UP \|_F \le \frac{ C\sqrt{d} \| A - P \| }{ \lambda_d(P) }.
\end{equation*}
%and thus
%\begin{equation*}
%\| \UA Q - \UP \|_F^2
%\le \frac{ C d \| A - P \|^2 }{ \lambda_d^2(P) }.
%\end{equation*}
Applying Equation~\ref{eq:specgrowth:2} yields~\eqref{eq:DKmodified}.
\end{proof}

\begin{lemma} \label{lem:frobnorm1}
With notation as above, letting 
$Q \in \bbR^{d \times d}$ denote the orthogonal matrix guaranteed by
Lemma~\ref{lem:2toinfty}, with probability at least $1-Cn^{-2}$,
\begin{equation*}
\| A\UA(\SA^{-1/2} Q -  Q\SP^{-1/2}) \|_F \le C n^{-1/2}.
%TODO: log factor?
%Again, depends on whether or not we are using Lu and Peng.
\end{equation*}
\end{lemma}
\begin{proof}
Let $E = A - \UA \SA \UA^T$ be the residual after making the best rank-$d$
approximation to $A$. By definition, the eigenvectors of $E$ are
orthogonal to the columns of $\UA$, whence $E \UA = 0$, and thus
$A \UA = \UA \SA$.
\begin{equation*}
\| A\UA(\SA^{-1/2} Q -  Q\SP^{-1/2}) \|_F
= \| \UA \SA \UA^T \UA (\SA^{-1/2} Q -  Q\SP^{-1/2}) \|_F
\le \| \SA \| \| \SA^{-1/2} Q - Q\SP^{-1/2} \|_F.
\end{equation*}
Lemma~\ref{lem:rdpgfacts} bounds the spectral norm as $O(n)$,
the Frobenius norm as $O(n^{-3/2})$, which completes the proof.
\end{proof}

The following lemma is a generalization of
Lemma 10 of \cite{LyzSusTanAthPri2014} to the
case where $\Delta = \E_F X_1 X_1^T \in \bbR^{d \times d}$ may have
repeated eigenvalues.
\begin{lemma} \label{lem:frobnorm2}
% Lemma 3.4 in arxiv: https://arxiv.org/pdf/1310.0532.pdf
% Lemma 10 in EJS: https://projecteuclid.org/download/pdfview_1/euclid.ejs/1420815881
With notation and setup as above,
Let $Q \in \bbR^{d \times d}$ be the orthogonal matrix guaranteed by
Lemma~\ref{lem:2toinfty}.
With probability at least $1-Cn^{-2}$,
\begin{equation*}
\| A(\UA Q - \UP)\SP^{-1/2} \|_F \le C n^{-1/2} \log n. %TODO: check log factor
\end{equation*}
\end{lemma}
\begin{proof}
Let $E = A - \UA \SA \UA^T$ as in the previous proof.
Taking $Q \in \bbR^{d \times d}$ to be as in Lemma~\ref{lem:2toinfty},
by the triangle inequality and basic properties of the Frobenius norm,
\begin{equation*} \begin{aligned}
\| A(\UA Q - \UP)\SP^{-1/2} \|_F
&= \| (\UA \SA \UA^T + E)(\UA Q - \UP) \SP^{-1/2} \|_F \\
&\le \| \UA \SA \| \| Q - \UA^T \UP \|_F \| \SP^{-1/2} \|
  + \| E \| \| \UA Q - \UP \|_F \| \SP^{-1/2} \|.
\end{aligned} \end{equation*}
Applying Lemma~\ref{lem:rdpgfacts},
with probability $1-Cn^{-2}$,
Equations~\eqref{eq:specgrowth:1} and~\eqref{eq:specgrowth:2},
both hold, so that
\begin{equation*}
\| \SP^{-1/2} \| = O(n^{-1/2}) \text{ and } \| \SA \| = O(n),
\end{equation*}
and Equation~\eqref{eq:innerprod} implies
\begin{equation*} \label{eq:Ugap:1}
\| \UA \| \| \SA \| \| Q - \UA^T \UP \|_F \| \SP^{-1/2} \|
% n n^{-1} \log n n^{-1/2}
\le  C n^{-1/2} \log n.
\end{equation*}
Similarly, since $\| E \| \le \|A-P\| = O(n^{1/2} \log n)$
by Equation~\eqref{eq:specgrowth:2},
Equation~\eqref{eq:DKmodified} implies that
\begin{equation*} \label{eq:Ugap:2}
\| E \| \| \UA Q - \UP \|_F \| \SP^{-1/2} \|
% n^{1/2} n^{-1/2} \log n n^{-1/2}
\le C n^{-1/2} \log n. %TODO: check log factor.
\end{equation*}
Thus, combining the above two displays,
\begin{equation*}
\| A(\UA Q - \UP)\SP^{-1/2} \|_F
\le C n^{-1/2} \log n, %TODO" log factor
\end{equation*}
as we set out to show.
\end{proof}




==> old_sbm_sp_expt.tex <==


We illustrate the full-network resampling scheme
discussed in Section~\ref{sec:netboot} on the problem of estimating the expected average shortest path length in a graph.
For a graph $G$ on $n$ vertices with adjacency matrix $A$,
the shortest path distance
between vertices $i$ and $j$, which we denote $d_A(i,j)$,
is given by the length of the shortest path connecting vertices $i$
and $j$ in $G$. We take $d_A(i,j) = \infty$ if $i$ and $j$ are in
different connected components.
The average shortest path distance,
\begin{equation} \label{eq:def:spdist}
\dbar_A = \binom{n}{2}^{-1} \sum_{i < j} d_A(i,j)
\end{equation}
provides a natural measure of the extent to which the graph
exhibits small-world behavior.
While at first glance Equation~\eqref{eq:def:spdist} appears to look like a U-statistic, this is not the case, since $d_A$ is a function that
itself depends on the data, not a fixed kernel.
To avoid the trivial case where $G$ is disconnected,
consider the problem of bootstrapping the quantity
\begin{equation*}
\E[ \dbar_A \mid \dbar_A < \infty].
\end{equation*}
The most natural approach to generating bootstrap samples of this quantity
is to generate bootstrap replicates of whole networks and evaluate this
quantity on each replicate.
The method introduced in Section~\ref{sec:netboot} is well-suited to this.

For comparison, we consider two other methods for generating network
bootstrap samples.
The first is an adaptation of the empirical graphon method
introduced by \cite{GreSha2017}.
In that paper, the authors considered producing bootstrap samples for subgraph
counts by, in essence, resampling vertices.
That is, one produces a bootstrap replicate adjacency matrix
$A^*$ by drawing $Z_1,Z_2,\dots,Z_n$ i.i.d.\ from the uniform distribution
on $[n]$, and take $A^*_{ij} = A_{Z_i,Z_j}$.
As acknowledged by the authors, a major drawback of this scheme
is that since the diagonal elements of $A$ are equal to $0$,
resampled vertices $k,\ell$ with $Z_k=Z_\ell$ are precluded
from forming an edge, which results in biased estimates of certain statistics.   For the purposes of estimating subgraph counts, this
drawback can be avoided, as demonstrated by the results in
\cite{GreSha2017}, but we will see that this causes a bias
when generating whole networks.
We suspect that correcting for this deficiency
is possible, but it is not trivial and we do not pursue the question here.
We also include, for the sake of comparison, a parametric bootstrap procedure, which performs estimation over a much smaller space of models
compared to the RDPG-based resampling scheme and the empirical graphon, and can thus serve as a gold standard when its underlying model is true.

In this set of experiments, following \cite{BhaBic2015}, % for number of vertices $n$,
we generate $A$ from a stochastic block model with two blocks and parameters
\begin{equation*}
B = B_n = \frac{5}{\sqrt{n}} \begin{bmatrix} 0.4 & 0.5 \\
                0.5 & 0.7 \end{bmatrix},
~~~\pi = \begin{bmatrix} 0.5 & 0.5 \end{bmatrix}.
\end{equation*}
%On each experiment trial, we generate an adjacency matrix $A \in \bbR^{n \times n}$ by drawing from an SBM with the above parameters,
We discard and regenerate $A$ in the event that it is not connected, since we are interested in the average shortest path in $A$ conditional on it being finite.
Given $A$, we construct the estimate $\Xhat = \ASE(A,2)$,
replacing the zeros on the diagonal of $A$ with the scaled degrees
$n^{-1} \sum_j A_{ij}$ as before.
Letting $\Fhat_n$ denote the empirical distribution of $\Xhat$,
we then draw $B=100$ bootstrap replicates of
$(\Ahat^*,\Xhat^*) \sim \RDPG( \Fhat_n, n )$,
computing the average shortest path of each iterate
(and resampling in the event that a sample $\Ahat^*$ is not connected).
We note that for finite $n$, the ASE may produce an estimate $\Xhat$
such that some entries of $\E[ \Ahat \mid \Xhat ] = \Xhat \Xhat^T$
are outside the interval [0,1].
When this occurs, we threshold the resulting
entries of the expected adjacency matrix to be either 0 or 1.
%That is, we define a Bernoulli random variable with negative success probability to be a point mass at $0$, and a Bernoulli random variable with success probability greater than $1$ to be a point mass at $1$.
For the empirical graphon procedure described above, we resample from the same original observed network $A$, resampling until a connected
graph is produced.
For the parametric bootstrap, we fit a 2-block SBM to the observed network
using spectral clustering.
Letting the estimated parameters be $(\Bhat,\pihat)$, we draw the $n \times n$ adjacentry matrix $\Ahat^*$ from  $\SBM( \Bhat, \pihat)$.
In all three bootstrap procedures, we generate $100$ bootstrap samples,
regenerating  as needed to ensure connected networks,
and use these $100$ bootstrap samples to obtain an estimate of the variance
of the average shortest path. We then use this variance to construct
a $95\%$ confidence interval centered on the observed
value of $\dbar_A$ via a normal approximation.

Letting the estimated parameters be $(\ahat,\bhat)$,                            we draw the $n \times n$ adjacentry matrix $\Ahat^*$ from
$\SBM( \Bhat, \pihat)$.
In all three bootstrap procedures, we generate $100$ bootstrap samples,
regenerating  as needed to ensure connected networks,
and use these $100$ bootstrap samples to obtain an estimate of the variance
of the average shortest path. We then use this variance to construct
a $95\%$ confidence interval centered on the observed
value of $\dbar_A$ via a normal approximation.

\begin{figure}[ht]
  \centering
  \subfloat[]{\includegraphics[width=0.5\columnwidth]{figs/SPSBM_CI_histogram.pdf}}
~~~
  \subfloat[]{\includegraphics[width=0.5\columnwidth]{figs/SPSBM_CI_singlerun.pdf}}
  \vspace{-3mm}
  \caption{(a) Bootstrap distributions produced by the different resampling schemes in a single trial,  $n=50$.
The plot shows smoothed density plots of $100$ samples of the average shortest path distance generated by the empirical graphon (Emp, red),
RDPG resampling (RDPG, blue), and the parametric bootstrap (Para, green). A sample of $100$ draws from the true model is also plotted (Truth, purple).
The black vertical line shows the estimated mean of the true distribution, based on 10,000 Monte Carlo samples.
(b) Confidence intervals produced based on the variances of the three different bootstrap samples for different values of $n$.
}
\label{fig:SPSBM:singlerun}
\end{figure}

For each of $n=50,100,200,500,1000$, we ran $200$ independent trials. % of the shortest paths experiment just described.
For illustration, results from a single run with $n=50$ are shown in Figure~\ref{fig:SPSBM:singlerun}.
Figure~\ref{fig:SPSBM:singlerun}(a) shows a smoothed density plot of the
$100$ bootstrap samples generated by the RDPG resampling scheme,
the empirical graphon and the parametric network bootstrap.
In addition, the plot shows the histogram of 100 independent draws
from the true distribution of the average shortest path under the generating model.
The black vertical line indicates the mean of this distribution,
estimated from 10,000 Monte Carlo samples, generated independently of the experimental trials.
It is clear from the plot that none of the three resampling methods captures
the true sampling distribution especially well,
though the parametric bootstrap gives a better approximation than
either the empirical graphon or the RDPG resampler.
Figure~\ref{fig:SPSBM:singlerun}(b) shows representative confidence intervals produced by
the three sampling methods for each choice of $n$, with the $n=50$ condition corresponding to the same trial as in (a).   We see that for this particular problem, the parametric
bootstrap scheme improves markedly over the other two methods,
yielding much narrower confidence intervals, as would be expected considering that the true model is in fact the SBM.

\begin{figure}[ht]
  \centering
  \subfloat[]{\includegraphics[width=0.5\columnwidth]{figs/SPSBM_CI_lengths.pdf}}
~~~
  \subfloat[]{\includegraphics[width=0.5\columnwidth]{figs/SPSBM_MSPbyNU.pdf}}
  \vspace{-3mm}
  \caption{(a) Average CI length over $200$ trials, for each value of $n$,
        produced by the empirical graphon (Emp, red),
        parametric bootstrap (Par, green) and
        RDPG resampler (RDPG, blue).
%       The parametric bootstrap consistently produced confidence       intervals about half the length of those produced by    the RDPG resampling scheme, and that the empirical graphon      produced confidence intervals that were wider still.  %LIZA - this belongs in the text, not the caption.  
        (b) Effect of scaling the average degree on the average shortest
        path length, for an SBM on $n=50,100,200$ vertices.}
  \label{fig:SPSBM:summary}
\end{figure}

This is further borne out in Figure~\ref{fig:SPSBM:summary}(a),
which shows the average confidence interval length over the $200$ trials,
for each of the three methods.
We see that the parametric bootstrap consistently gives a confidence interval
approximately half as long as that constructed by the RDPG sampling scheme,
and that the empirical graphon performs still worse.
Unsurprisingly, given the widths of the confidence intervals,
the coverage rates of both the RDPG and empirical graphon were both
uniformly $1$,
while the parametric bootstrap had an estimated coverage rate that
varied between 0.93 and 0.96 across the five values of $n$.
We note that since the true expected average shortest path distance
is estimated via Monte Carlo, we computed coverage rates under
the milder requirement that a confidence interval was considered to have
covered the target if it overlapped the interval comprising
two standard errors of the mean of the Monte Carlo samples.
This adjustment did not appreciably change the coverage rates of the
RDPG or empirical empirical graphon, but was required in order to obtain the (approximately) correct coverage rate for the parametric bootstrap.

Figure~\ref{fig:SPSBM:summary}(b) helps to illustrate the challenge of this problem. Consider rescaling the matrix $B$ in the SBM described above with
\begin{equation*}
B_\nu = \frac{ \nu }{ \sqrt{n} } \begin{bmatrix} 0.4 & 0.5 \\
                0.5 & 0.7 \end{bmatrix}.
\end{equation*}
%LIZA: Not important, but $\nu$ was already used for something else, this could be $\lambda$. 
%KEITH: I'll fix this in the journal version,-- fixing this here will require also regenerating the plots.
As $\nu$ increases, the number of edges increases on average, and thus
the shortest paths between vertices tend to become shorter.
%As $\nu$ decreases, there are fewer edges in the network on average, and shortest paths become longer.
Figure~\ref{fig:SPSBM:summary}(b) plots the average
shortest path distance as a function of $\nu$ for different values of $n$,
%Each line is based on point estimates of the average shortest path distance, with each estimate 
based on $100$ Monte Carlo replicates from
$\SBM( B_\nu, \pi )$.
The shaded region indicates two standard errors of the mean.
We see that, especially for sparser networks, a comparatively small change in the parameter $\nu$ may result in an outsized effect on the average shortest path length.  While this does not pose a severe problem for the parametric bootstrap, since the variance as a function of $\nu$ does not change nearly as quickly
as the average shortest path length, we suspect that it does
partially explain the overly wide confidence intervals produced by
the RDPG resampling scheme.
Variance in the expected degree of $\E[ \Ahat^* \mid \Xhat^* ]$
in turn results in higher variance in the average shotrest path length.
 %LIZA:  I am not entirely sure that this is the reason it breaks down... it seems more likely to me it's just that resampling from the correct parametric model cannot be beat.  Leaving it in though in case you somehow know that this is the reason.  
 %KEITH: I have rewritten to be more clear about why I think this is the reason.jj






